Parallel lives: A local-realistic interpretation of "nonlocal" boxes

We carry out a thought experiment in an imaginary world. Our world is both local and realistic, yet it violates a Bell inequality more than does quantum theory. This serves to debunk the myth that equates local realism with local hidden variables in the simplest possible manner. Along the way, we reinterpret the celebrated 1935 argument of Einstein, Podolsky and Rosen, and come to the conclusion that they were right in their questioning the completeness of the Copenhagen version of quantum theory, provided one believes in a local-realistic universe. Throughout our journey, we strive to explain our views from first principles, without expecting mathematical sophistication nor specialized prior knowledge from the reader.

==> Definitions/journalnames.tex <==
\DeclareOption{acoustics}{	\gdef\@journal{acoustics}	\gdef\@journalshort{Acoustics}	\gdef\@journalfull{Acoustics}	\gdef\@doiabbr{acoustics}	\gdef\@ISSN{2624-599X}	}
\DeclareOption{actuators}{	\gdef\@journal{actuators}	\gdef\@journalshort{Actuators}	\gdef\@journalfull{Actuators}	\gdef\@doiabbr{act}	\gdef\@ISSN{2076-0825}	}
\DeclareOption{addictions}{	\gdef\@journal{addictions}	\gdef\@journalshort{Addictions}	\gdef\@journalfull{Addictions}	\gdef\@doiabbr{}	\gdef\@ISSN{0006-0006}	}
\DeclareOption{admsci}{	\gdef\@journal{admsci}	\gdef\@journalshort{Adm. Sci.}	\gdef\@journalfull{Administrative Sciences}	\gdef\@doiabbr{admsci}	\gdef\@ISSN{2076-3387}	}
\DeclareOption{aerospace}{	\gdef\@journal{aerospace}	\gdef\@journalshort{Aerospace}	\gdef\@journalfull{Aerospace}	\gdef\@doiabbr{aerospace}	\gdef\@ISSN{2226-4310}	}
\DeclareOption{agriculture}{	\gdef\@journal{agriculture}	\gdef\@journalshort{Agriculture}	\gdef\@journalfull{Agriculture}	\gdef\@doiabbr{agriculture}	\gdef\@ISSN{2077-0472}	}
\DeclareOption{agriengineering}{	\gdef\@journal{agriengineering}	\gdef\@journalshort{AgriEngineering}	\gdef\@journalfull{AgriEngineering}	\gdef\@doiabbr{}	\gdef\@ISSN{}	}
\DeclareOption{agronomy}{	\gdef\@journal{agronomy}	\gdef\@journalshort{Agronomy}	\gdef\@journalfull{Agronomy}	\gdef\@doiabbr{agronomy}	\gdef\@ISSN{2073-4395}	}
\DeclareOption{algorithms}{	\gdef\@journal{algorithms}	\gdef\@journalshort{Algorithms}	\gdef\@journalfull{Algorithms}	\gdef\@doiabbr{a}	\gdef\@ISSN{1999-4893}	}
\DeclareOption{animals}{	\gdef\@journal{animals}	\gdef\@journalshort{Animals}	\gdef\@journalfull{Animals}	\gdef\@doiabbr{ani}	\gdef\@ISSN{2076-2615}	}
\DeclareOption{antibiotics}{	\gdef\@journal{antibiotics}	\gdef\@journalshort{Antibiotics}	\gdef\@journalfull{Antibiotics}	\gdef\@doiabbr{antibiotics}	\gdef\@ISSN{2079-6382}	}
\DeclareOption{antibodies}{	\gdef\@journal{antibodies}	\gdef\@journalshort{Antibodies}	\gdef\@journalfull{Antibodies}	\gdef\@doiabbr{antib}	\gdef\@ISSN{2073-4468}	}
\DeclareOption{antioxidants}{	\gdef\@journal{antioxidants}	\gdef\@journalshort{Antioxidants}	\gdef\@journalfull{Antioxidants}	\gdef\@doiabbr{antiox}	\gdef\@ISSN{2076-3921}	}
\DeclareOption{applsci}{	\gdef\@journal{applsci}	\gdef\@journalshort{Appl. Sci.}	\gdef\@journalfull{Applied Sciences}	\gdef\@doiabbr{app}	\gdef\@ISSN{2076-3417}	}
\DeclareOption{arts}{	\gdef\@journal{arts}	\gdef\@journalshort{Arts}	\gdef\@journalfull{Arts}	\gdef\@doiabbr{arts}	\gdef\@ISSN{2076-0752}	}
\DeclareOption{asi}{	\gdef\@journal{asi}	\gdef\@journalshort{Appl. Syst. Innov.}	\gdef\@journalfull{Applied System Innovation}	\gdef\@doiabbr{asi}	\gdef\@ISSN{2571-5577}	}
\DeclareOption{atmosphere}{	\gdef\@journal{atmosphere}	\gdef\@journalshort{Atmosphere}	\gdef\@journalfull{Atmosphere}	\gdef\@doiabbr{atmos}	\gdef\@ISSN{2073-4433}	}
\DeclareOption{atoms}{	\gdef\@journal{atoms}	\gdef\@journalshort{Atoms}	\gdef\@journalfull{Atoms}	\gdef\@doiabbr{atoms}	\gdef\@ISSN{2218-2004}	}
\DeclareOption{axioms}{	\gdef\@journal{axioms}	\gdef\@journalshort{Axioms}	\gdef\@journalfull{Axioms}	\gdef\@doiabbr{axioms}	\gdef\@ISSN{2075-1680}	}
\DeclareOption{batteries}{	\gdef\@journal{batteries}	\gdef\@journalshort{Batteries}	\gdef\@journalfull{Batteries}	\gdef\@doiabbr{batteries}	\gdef\@ISSN{2313-0105}	}
\DeclareOption{bdcc}{	\gdef\@journal{bdcc}	\gdef\@journalshort{Big Data Cogn. Comput.}	\gdef\@journalfull{Big Data and Cognitive Computing}	\gdef\@doiabbr{bdcc}	\gdef\@ISSN{2504-2289}	}
\DeclareOption{behavsci}{ 	\gdef\@journal{behavsci} 	\gdef\@journalshort{Behav. Sci.}	\gdef\@journalfull{Behavioral Sciences}	\gdef\@doiabbr{bs}	\gdef\@ISSN{2076-328X}	}
\DeclareOption{beverages}{	\gdef\@journal{beverages}	\gdef\@journalshort{Beverages}	\gdef\@journalfull{Beverages}	\gdef\@doiabbr{beverages}	\gdef\@ISSN{2306-5710}	}
\DeclareOption{bioengineering}{	\gdef\@journal{bioengineering}	\gdef\@journalshort{Bioengineering}	\gdef\@journalfull{Bioengineering}	\gdef\@doiabbr{bioengineering}	\gdef\@ISSN{2306-5354}	}
\DeclareOption{biology}{	\gdef\@journal{biology}	\gdef\@journalshort{Biology}	\gdef\@journalfull{Biology}	\gdef\@doiabbr{biology}	\gdef\@ISSN{2079-7737}	}
\DeclareOption{biomedicines}{	\gdef\@journal{biomedicines}	\gdef\@journalshort{Biomedicines}	\gdef\@journalfull{Biomedicines}	\gdef\@doiabbr{biomedicines}	\gdef\@ISSN{2227-9059}	}
\DeclareOption{biomimetics}{	\gdef\@journal{biomimetics}	\gdef\@journalshort{Biomimetics}	\gdef\@journalfull{Biomimetics}	\gdef\@doiabbr{biomimetics}	\gdef\@ISSN{2313-7673}	}
\DeclareOption{biomolecules}{	\gdef\@journal{biomolecules}	\gdef\@journalshort{Biomolecules}	\gdef\@journalfull{Biomolecules}	\gdef\@doiabbr{biom}	\gdef\@ISSN{2218-273X}	}
\DeclareOption{biosensors}{	\gdef\@journal{biosensors}	\gdef\@journalshort{Biosensors}	\gdef\@journalfull{Biosensors}	\gdef\@doiabbr{bios}	\gdef\@ISSN{2079-6374}	}
\DeclareOption{brainsci}{ 	\gdef\@journal{brainsci} 	\gdef\@journalshort{Brain Sci.}	\gdef\@journalfull{Brain Sciences}	\gdef\@doiabbr{brainsci}	\gdef\@ISSN{2076-3425}	}
\DeclareOption{buildings}{	\gdef\@journal{buildings}	\gdef\@journalshort{Buildings}	\gdef\@journalfull{Buildings}	\gdef\@doiabbr{buildings}	\gdef\@ISSN{2075-5309}	}
\DeclareOption{cancers}{	\gdef\@journal{cancers}	\gdef\@journalshort{Cancers}	\gdef\@journalfull{Cancers}	\gdef\@doiabbr{cancers}	\gdef\@ISSN{2072-6694}	}
\DeclareOption{carbon}{ 	\gdef\@journal{carbon} 	\gdef\@journalshort{C}	\gdef\@journalfull{C}	\gdef\@doiabbr{c}	\gdef\@ISSN{2311-5629}	}
\DeclareOption{catalysts}{	\gdef\@journal{catalysts}	\gdef\@journalshort{Catalysts}	\gdef\@journalfull{Catalysts}	\gdef\@doiabbr{catal}	\gdef\@ISSN{2073-4344}	}
\DeclareOption{cells}{	\gdef\@journal{cells}	\gdef\@journalshort{Cells}	\gdef\@journalfull{Cells}	\gdef\@doiabbr{cells}	\gdef\@ISSN{2073-4409}	}
\DeclareOption{ceramics}{	\gdef\@journal{ceramics}	\gdef\@journalshort{Ceramics}	\gdef\@journalfull{Ceramics}	\gdef\@doiabbr{ceramics}	\gdef\@ISSN{2571-6131}	}
\DeclareOption{challenges}{	\gdef\@journal{challenges}	\gdef\@journalshort{Challenges}	\gdef\@journalfull{Challenges}	\gdef\@doiabbr{challe}	\gdef\@ISSN{2078-1547}	}
\DeclareOption{chemengineering}{	\gdef\@journal{chemengineering}	\gdef\@journalshort{ChemEngineering}	\gdef\@journalfull{ChemEngineering}	\gdef\@doiabbr{chemengineering}	\gdef\@ISSN{2305-7084}	}
\DeclareOption{chemosensors}{	\gdef\@journal{chemosensors}	\gdef\@journalshort{Chemosensors}	\gdef\@journalfull{Chemosensors}	\gdef\@doiabbr{chemosensors}	\gdef\@ISSN{2227-9040}	}
\DeclareOption{children}{	\gdef\@journal{children}	\gdef\@journalshort{Children}	\gdef\@journalfull{Children}	\gdef\@doiabbr{children}	\gdef\@ISSN{2227-9067}	}
\DeclareOption{cleantechnol}{	\gdef\@journal{cleantechnol}	\gdef\@journalshort{Clean Technol.}	\gdef\@journalfull{Clean Technologies}	\gdef\@doiabbr{cleantechnol}	\gdef\@ISSN{2571-8797}	}
\DeclareOption{climate}{	\gdef\@journal{climate}	\gdef\@journalshort{Climate}	\gdef\@journalfull{Climate}	\gdef\@doiabbr{cli}	\gdef\@ISSN{2225-1154}	}
\DeclareOption{clockssleep}{	\gdef\@journal{clockssleep}	\gdef\@journalshort{Clocks\&Sleep}	\gdef\@journalfull{Clocks \& Sleep}	\gdef\@doiabbr{clockssleep}	\gdef\@ISSN{2624-5175}	}
\DeclareOption{cmd}{	\gdef\@journal{cmd}	\gdef\@journalshort{Corros. Mater. Degrad.}	\gdef\@journalfull{Corrosion and Materials Degradation}	\gdef\@doiabbr{cmd}	\gdef\@ISSN{2624-5558}	}
\DeclareOption{coatings}{	\gdef\@journal{coatings}	\gdef\@journalshort{Coatings}	\gdef\@journalfull{Coatings}	\gdef\@doiabbr{coatings}	\gdef\@ISSN{2079-6412}	}
\DeclareOption{colloids}{	\gdef\@journal{colloids}	\gdef\@journalshort{Colloids Interfaces}	\gdef\@journalfull{Colloids Interfaces}	\gdef\@doiabbr{colloids}	\gdef\@ISSN{2504-5377}	}
\DeclareOption{computation}{	\gdef\@journal{computation}	\gdef\@journalshort{Computation}	\gdef\@journalfull{Computation}	\gdef\@doiabbr{computation}	\gdef\@ISSN{2079-3197}	}
\DeclareOption{computers}{	\gdef\@journal{computers}	\gdef\@journalshort{Computers}	\gdef\@journalfull{Computers}	\gdef\@doiabbr{computers}	\gdef\@ISSN{2073-431X}	}
\DeclareOption{condensedmatter}{	\gdef\@journal{condensedmatter}	\gdef\@journalshort{Condens. Matter}	\gdef\@journalfull{Condensed Matter}	\gdef\@doiabbr{condmat}	\gdef\@ISSN{2410-3896}	}
\DeclareOption{cosmetics}{	\gdef\@journal{cosmetics}	\gdef\@journalshort{Cosmetics}	\gdef\@journalfull{Cosmetics}	\gdef\@doiabbr{cosmetics}	\gdef\@ISSN{2079-9284}	}
\DeclareOption{cryptography}{	\gdef\@journal{cryptography}	\gdef\@journalshort{Cryptography}	\gdef\@journalfull{Cryptography}	\gdef\@doiabbr{cryptography}	\gdef\@ISSN{2410-387X}	}
\DeclareOption{crystals}{	\gdef\@journal{crystals}	\gdef\@journalshort{Crystals}	\gdef\@journalfull{Crystals}	\gdef\@doiabbr{cryst}	\gdef\@ISSN{2073-4352}	}
\DeclareOption{cybersecurity}{	\gdef\@journal{cybersecurity}	\gdef\@journalshort{Cybersecurity}	\gdef\@journalfull{Cybersecurity}	\gdef\@doiabbr{cybersecurity}	\gdef\@ISSN{2624-800X}	}
\DeclareOption{dairy}{	\gdef\@journal{dairy}	\gdef\@journalshort{Dairy}	\gdef\@journalfull{Dairy}	\gdef\@doiabbr{dairy}	\gdef\@ISSN{2624-862X}	}
\DeclareOption{data}{	\gdef\@journal{data}	\gdef\@journalshort{Data}	\gdef\@journalfull{Data}	\gdef\@doiabbr{data}	\gdef\@ISSN{2306-5729}	}
\DeclareOption{dentistry}{	\gdef\@journal{dentistry}	\gdef\@journalshort{Dent. J.}	\gdef\@journalfull{Dentistry Journal}	\gdef\@doiabbr{dj}	\gdef\@ISSN{2304-6767}	}
\DeclareOption{designs}{ 	\gdef\@journal{designs} 	\gdef\@journalshort{Designs}	\gdef\@journalfull{Designs}	\gdef\@doiabbr{designs}	\gdef\@ISSN{2411-9660}	}
\DeclareOption{diagnostics}{	\gdef\@journal{diagnostics}	\gdef\@journalshort{Diagnostics}	\gdef\@journalfull{Diagnostics}	\gdef\@doiabbr{diagnostics}	\gdef\@ISSN{2075-4418}	}
\DeclareOption{diseases}{	\gdef\@journal{diseases}	\gdef\@journalshort{Diseases}	\gdef\@journalfull{Diseases}	\gdef\@doiabbr{diseases}	\gdef\@ISSN{2079-9721}	}
\DeclareOption{diversity}{	\gdef\@journal{diversity}	\gdef\@journalshort{Diversity}	\gdef\@journalfull{Diversity}	\gdef\@doiabbr{d}	\gdef\@ISSN{1424-2818}	}
\DeclareOption{drones}{	\gdef\@journal{drones}	\gdef\@journalshort{Drones}	\gdef\@journalfull{Drones}	\gdef\@doiabbr{drones}	\gdef\@ISSN{2504-446X}	}
\DeclareOption{econometrics}{	\gdef\@journal{econometrics}	\gdef\@journalshort{Econometrics}	\gdef\@journalfull{Econometrics}	\gdef\@doiabbr{econometrics}	\gdef\@ISSN{2225-1146}	}
\DeclareOption{economies}{	\gdef\@journal{economies}	\gdef\@journalshort{Economies}	\gdef\@journalfull{Economies}	\gdef\@doiabbr{economies}	\gdef\@ISSN{2227-7099}	}
\DeclareOption{education}{	\gdef\@journal{education}	\gdef\@journalshort{Educ. Sci.}	\gdef\@journalfull{Education Sciences}	\gdef\@doiabbr{educsci}	\gdef\@ISSN{2227-7102}	}
\DeclareOption{electrochem}{	\gdef\@journal{electrochem}	\gdef\@journalshort{Electrochem}	\gdef\@journalfull{Electrochem}	\gdef\@doiabbr{electrochem}	\gdef\@ISSN{}	}
\DeclareOption{electronics}{	\gdef\@journal{electronics}	\gdef\@journalshort{Electronics}	\gdef\@journalfull{Electronics}	\gdef\@doiabbr{electronics}	\gdef\@ISSN{2079-9292}	}
\DeclareOption{energies}{	\gdef\@journal{energies}	\gdef\@journalshort{Energies}	\gdef\@journalfull{Energies}	\gdef\@doiabbr{en}	\gdef\@ISSN{1996-1073}	}
\DeclareOption{entropy}{	\gdef\@journal{entropy}	\gdef\@journalshort{Entropy}	\gdef\@journalfull{Entropy}	\gdef\@doiabbr{e}	\gdef\@ISSN{1099-4300}	}
\DeclareOption{environments}{	\gdef\@journal{environments}	\gdef\@journalshort{Environments}	\gdef\@journalfull{Environments}	\gdef\@doiabbr{environments}	\gdef\@ISSN{2076-3298}	}
\DeclareOption{epigenomes}{	\gdef\@journal{epigenomes}	\gdef\@journalshort{Epigenomes}	\gdef\@journalfull{Epigenomes}	\gdef\@doiabbr{epigenomes}	\gdef\@ISSN{2075-4655}	}
\DeclareOption{est}{	\gdef\@journal{est}	\gdef\@journalshort{Electrochem. Sci. Technol.}	\gdef\@journalfull{Electrochemical Science and Technology}	\gdef\@doiabbr{}	\gdef\@ISSN{}	}
\DeclareOption{fermentation}{	\gdef\@journal{fermentation}	\gdef\@journalshort{Fermentation}	\gdef\@journalfull{Fermentation}	\gdef\@doiabbr{fermentation}	\gdef\@ISSN{2311-5637}	}
\DeclareOption{fibers}{	\gdef\@journal{fibers}	\gdef\@journalshort{Fibers}	\gdef\@journalfull{Fibers}	\gdef\@doiabbr{fib}	\gdef\@ISSN{2079-6439}	}
\DeclareOption{fire}{	\gdef\@journal{fire}	\gdef\@journalshort{Fire}	\gdef\@journalfull{Fire}	\gdef\@doiabbr{fire}	\gdef\@ISSN{2571-6255}	}
\DeclareOption{fishes}{	\gdef\@journal{fishes}	\gdef\@journalshort{Fishes}	\gdef\@journalfull{Fishes}	\gdef\@doiabbr{fishes}	\gdef\@ISSN{2410-3888}	}
\DeclareOption{fluids}{	\gdef\@journal{fluids}	\gdef\@journalshort{Fluids}	\gdef\@journalfull{Fluids}	\gdef\@doiabbr{fluids}	\gdef\@ISSN{2311-5521}	}
\DeclareOption{foods}{	\gdef\@journal{foods}	\gdef\@journalshort{Foods}	\gdef\@journalfull{Foods}	\gdef\@doiabbr{foods}	\gdef\@ISSN{2304-8158}	}
\DeclareOption{forecasting}{	\gdef\@journal{forecasting}	\gdef\@journalshort{Forecasting}	\gdef\@journalfull{Forecasting}	\gdef\@doiabbr{forecast}	\gdef\@ISSN{2571-9394}	}
\DeclareOption{forests}{	\gdef\@journal{forests}	\gdef\@journalshort{Forests}	\gdef\@journalfull{Forests}	\gdef\@doiabbr{f}	\gdef\@ISSN{1999-4907}	}
\DeclareOption{fractalfract}{	\gdef\@journal{fractalfract}	\gdef\@journalshort{Fractal Fract.}	\gdef\@journalfull{Fractal and Fractional}	\gdef\@doiabbr{fractalfract}	\gdef\@ISSN{2504-3110}	}
\DeclareOption{futureinternet}{	\gdef\@journal{futureinternet}	\gdef\@journalshort{Future Internet}	\gdef\@journalfull{Future Internet}	\gdef\@doiabbr{fi}	\gdef\@ISSN{1999-5903}	}
\DeclareOption{galaxies}{	\gdef\@journal{galaxies}	\gdef\@journalshort{Galaxies}	\gdef\@journalfull{Galaxies}	\gdef\@doiabbr{galaxies}	\gdef\@ISSN{2075-4434}	}
\DeclareOption{games}{	\gdef\@journal{games}	\gdef\@journalshort{Games}	\gdef\@journalfull{Games}	\gdef\@doiabbr{g}	\gdef\@ISSN{2073-4336}	}
\DeclareOption{gastrointestdisord}{	\gdef\@journal{gastrointestdisord}	\gdef\@journalshort{Gastrointest. Disord.}	\gdef\@journalfull{Gastrointestinal Disorders}	\gdef\@doiabbr{gidisord}	\gdef\@ISSN{2624-5647}	}
\DeclareOption{gels}{	\gdef\@journal{gels}	\gdef\@journalshort{Gels}	\gdef\@journalfull{Gels}	\gdef\@doiabbr{gels}	\gdef\@ISSN{2310-2861}	}
\DeclareOption{genealogy}{	\gdef\@journal{genealogy}	\gdef\@journalshort{Genealogy}	\gdef\@journalfull{Genealogy}	\gdef\@doiabbr{genealogy}	\gdef\@ISSN{2313-5778}	}
\DeclareOption{genes}{	\gdef\@journal{genes}	\gdef\@journalshort{Genes}	\gdef\@journalfull{Genes}	\gdef\@doiabbr{genes}	\gdef\@ISSN{2073-4425}	}
\DeclareOption{geohazards}{	\gdef\@journal{geohazards}	\gdef\@journalshort{GeoHazards}	\gdef\@journalfull{GeoHazards}	\gdef\@doiabbr{geohazards}	\gdef\@ISSN{2624-795X}	}
\DeclareOption{geosciences}{	\gdef\@journal{geosciences}	\gdef\@journalshort{Geosciences}	\gdef\@journalfull{Geosciences}	\gdef\@doiabbr{geosciences}	\gdef\@ISSN{2076-3263}	}
\DeclareOption{geriatrics}{	\gdef\@journal{geriatrics}	\gdef\@journalshort{Geriatrics}	\gdef\@journalfull{Geriatrics}	\gdef\@doiabbr{geriatrics}	\gdef\@ISSN{2308-3417}	}
\DeclareOption{hazardousmatters}{	\gdef\@journal{hazardousmatters}	\gdef\@journalshort{Hazard. Matters}	\gdef\@journalfull{Hazardous Matters}	\gdef\@doiabbr{}	\gdef\@ISSN{0014-0014}	}
\DeclareOption{healthcare}{	\gdef\@journal{healthcare}	\gdef\@journalshort{Healthcare}	\gdef\@journalfull{Healthcare}	\gdef\@doiabbr{healthcare}	\gdef\@ISSN{2227-9032}	}
\DeclareOption{heritage}{	\gdef\@journal{heritage}	\gdef\@journalshort{Heritage}	\gdef\@journalfull{Heritage}	\gdef\@doiabbr{heritage}	\gdef\@ISSN{2571-9408}	}
\DeclareOption{highthroughput}{	\gdef\@journal{highthroughput}	\gdef\@journalshort{High-Throughput}	\gdef\@journalfull{High-Throughput}	\gdef\@doiabbr{ht}	\gdef\@ISSN{2571-5135}	}
\DeclareOption{horticulturae}{	\gdef\@journal{horticulturae}	\gdef\@journalshort{Horticulturae}	\gdef\@journalfull{Horticulturae}	\gdef\@doiabbr{horticulturae}	\gdef\@ISSN{2311-7524}	}
\DeclareOption{humanities}{	\gdef\@journal{humanities}	\gdef\@journalshort{Humanities}	\gdef\@journalfull{Humanities}	\gdef\@doiabbr{h}	\gdef\@ISSN{2076-0787}	}
\DeclareOption{hydrology}{	\gdef\@journal{hydrology}	\gdef\@journalshort{Hydrology}	\gdef\@journalfull{Hydrology}	\gdef\@doiabbr{hydrology}	\gdef\@ISSN{2306-5338}	}
\DeclareOption{ijerph}{	\gdef\@journal{ijerph}	\gdef\@journalshort{Int. J. Environ. Res. Public Health}	\gdef\@journalfull{International Journal of Environmental Research and Public Health}	\gdef\@doiabbr{ijerph}	\gdef\@ISSN{1660-4601}	}
\DeclareOption{ijfs}{	\gdef\@journal{ijfs}	\gdef\@journalshort{Int. J. Financial Stud.}	\gdef\@journalfull{International Journal of Financial Studies}	\gdef\@doiabbr{ijfs}	\gdef\@ISSN{2227-7072}	}
\DeclareOption{ijgi}{	\gdef\@journal{ijgi}	\gdef\@journalshort{ISPRS Int. J. Geo-Inf.}	\gdef\@journalfull{ISPRS International Journal of Geo-Information}	\gdef\@doiabbr{ijgi}	\gdef\@ISSN{2220-9964}	}
\DeclareOption{ijms}{	\gdef\@journal{ijms}	\gdef\@journalshort{Int. J. Mol. Sci.}	\gdef\@journalfull{International Journal of Molecular Sciences}	\gdef\@doiabbr{ijms}	\gdef\@ISSN{1422-0067}	}
\DeclareOption{ijtpp}{	\gdef\@journal{ijtpp}	\gdef\@journalshort{Int. J. Turbomach. Propuls. Power}	"\gdef\@journalfull{International Journal of Turbomachinery, Propulsion and Power}"	\gdef\@doiabbr{ijtpp}	\gdef\@ISSN{2504-186X}	}
\DeclareOption{informatics}{	\gdef\@journal{informatics}	\gdef\@journalshort{Informatics}	\gdef\@journalfull{Informatics}	\gdef\@doiabbr{informatics}	\gdef\@ISSN{2227-9709}	}
\DeclareOption{information}{	\gdef\@journal{information}	\gdef\@journalshort{Information}	\gdef\@journalfull{Information}	\gdef\@doiabbr{info}	\gdef\@ISSN{2078-2489}	}
\DeclareOption{infrastructures}{	\gdef\@journal{infrastructures}	\gdef\@journalshort{Infrastructures}	\gdef\@journalfull{Infrastructures}	\gdef\@doiabbr{infrastructures}	\gdef\@ISSN{2412-3811}	}
\DeclareOption{inorganics}{	\gdef\@journal{inorganics}	\gdef\@journalshort{Inorganics}	\gdef\@journalfull{Inorganics}	\gdef\@doiabbr{inorganics}	\gdef\@ISSN{2304-6740}	}
\DeclareOption{insects}{	\gdef\@journal{insects}	\gdef\@journalshort{Insects}	\gdef\@journalfull{Insects}	\gdef\@doiabbr{insects}	\gdef\@ISSN{2075-4450}	}
\DeclareOption{instruments}{	\gdef\@journal{instruments}	\gdef\@journalshort{Instruments}	\gdef\@journalfull{Instruments}	\gdef\@doiabbr{instruments}	\gdef\@ISSN{2410-390X}	}
\DeclareOption{inventions}{	\gdef\@journal{inventions}	\gdef\@journalshort{Inventions}	\gdef\@journalfull{Inventions}	\gdef\@doiabbr{inventions}	\gdef\@ISSN{2411-5134}	}
\DeclareOption{iot}{	\gdef\@journal{iot}	\gdef\@journalshort{IoT}	\gdef\@journalfull{IoT}	\gdef\@doiabbr{iot}	\gdef\@ISSN{2624-831X}	}
\DeclareOption{j}{	\gdef\@journal{jjournal}	\gdef\@journalshort{J}	\gdef\@journalfull{J}	\gdef\@doiabbr{j}	\gdef\@ISSN{2571-8800}	}
\DeclareOption{jcdd}{	\gdef\@journal{jcdd}	\gdef\@journalshort{J. Cardiovasc. Dev. Dis.}	\gdef\@journalfull{Journal of Cardiovascular Development and Disease}	\gdef\@doiabbr{jcdd}	\gdef\@ISSN{2308-3425}	}
\DeclareOption{jcm}{	\gdef\@journal{jcm}	\gdef\@journalshort{J. Clin. Med.}	\gdef\@journalfull{Journal of Clinical Medicine}	\gdef\@doiabbr{jcm}	\gdef\@ISSN{2077-0383}	}
\DeclareOption{jcs}{	\gdef\@journal{jcs}	\gdef\@journalshort{J. Compos. Sci.}	\gdef\@journalfull{Journal of Composites Science}	\gdef\@doiabbr{jcs}	\gdef\@ISSN{2504-477X}	}
\DeclareOption{jdb}{	\gdef\@journal{jdb}	\gdef\@journalshort{J. Dev. Biol.}	\gdef\@journalfull{Journal of Developmental Biology}	\gdef\@doiabbr{jdb}	\gdef\@ISSN{2221-3759}	}
\DeclareOption{jfb}{	\gdef\@journal{jfb}	\gdef\@journalshort{J. Funct. Biomater.}   	\gdef\@journalfull{Journal of Functional Biomaterials}   	\gdef\@doiabbr{jfb}	\gdef\@ISSN{2079-4983}	}
\DeclareOption{jfmk}{	\gdef\@journal{jfmk}	\gdef\@journalshort{J. Funct. Morphol. Kinesiol.}   	\gdef\@journalfull{Journal of Functional Morphology and Kinesiology}   	\gdef\@doiabbr{jfmk}	\gdef\@ISSN{2411-5142}	}
\DeclareOption{jimaging}{	\gdef\@journal{jimaging}	\gdef\@journalshort{J. Imaging}	\gdef\@journalfull{Journal of Imaging}	\gdef\@doiabbr{jimaging}	\gdef\@ISSN{2313-433X}	}
\DeclareOption{jintelligence}{	\gdef\@journal{jintelligence}	\gdef\@journalshort{J. Intell.}	\gdef\@journalfull{Journal of Intelligence}	\gdef\@doiabbr{jintelligence}	\gdef\@ISSN{2079-3200}	}
\DeclareOption{jlpea}{	\gdef\@journal{jlpea}	\gdef\@journalshort{J. Low Power Electron. Appl.}	\gdef\@journalfull{Journal of Low Power Electronics and Applications}	\gdef\@doiabbr{jlpea}	\gdef\@ISSN{2079-9268}	}
\DeclareOption{jmmp}{	\gdef\@journal{jmmp}	\gdef\@journalshort{J. Manuf. Mater. Process.}	\gdef\@journalfull{Journal of Manufacturing and Materials Processing}	\gdef\@doiabbr{jmmp}	\gdef\@ISSN{2504-4494}	}
\DeclareOption{jmse}{	\gdef\@journal{jmse}	\gdef\@journalshort{J. Mar. Sci. Eng.}	\gdef\@journalfull{Journal of Marine Science and Engineering}	\gdef\@doiabbr{jmse}	\gdef\@ISSN{2077-1312}	}
\DeclareOption{jnt}{	\gdef\@journal{jnt}	\gdef\@journalshort{J. Nanotheranostics}	\gdef\@journalfull{Journal of Nanotheranostics}	\gdef\@doiabbr{}	\gdef\@ISSN{}	}
\DeclareOption{jof}{	\gdef\@journal{jof}	\gdef\@journalshort{J. Fungi}	\gdef\@journalfull{Journal of Fungi}	\gdef\@doiabbr{jof}	\gdef\@ISSN{2309-608X}	}
\DeclareOption{joitmc}{	\gdef\@journal{joitmc}	\gdef\@journalshort{J. Open Innov. Technol. Mark. Complex.}	"\gdef\@journalfull{Journal of Open Innovation: Technology, Market, and Complexity}"	\gdef\@doiabbr{joitmc}	\gdef\@ISSN{2199-8531}	}
\DeclareOption{jpm}{	\gdef\@journal{jpm}	\gdef\@journalshort{J. Pers. Med.}	\gdef\@journalfull{Journal of Personalized Medicine}	\gdef\@doiabbr{jpm}	\gdef\@ISSN{2075-4426}	}
\DeclareOption{jrfm}{	\gdef\@journal{jrfm}	\gdef\@journalshort{J. Risk Financial Manag.}	\gdef\@journalfull{Journal of Risk and Financial Management}	\gdef\@doiabbr{jrfm}	\gdef\@ISSN{1911-8074}	}
\DeclareOption{jsan}{	\gdef\@journal{jsan}	\gdef\@journalshort{J. Sens. Actuator Netw.}	\gdef\@journalfull{Journal of Sensor and Actuator Networks}	\gdef\@doiabbr{jsan}	\gdef\@ISSN{2224-2708}	}
\DeclareOption{land}{	\gdef\@journal{land}	\gdef\@journalshort{Land}	\gdef\@journalfull{Land}	\gdef\@doiabbr{land}	\gdef\@ISSN{2073-445X}	}
\DeclareOption{languages}{	\gdef\@journal{languages}	\gdef\@journalshort{Languages}	\gdef\@journalfull{Languages}	\gdef\@doiabbr{languages}	\gdef\@ISSN{2226-471X}	}
\DeclareOption{laws}{	\gdef\@journal{laws}	\gdef\@journalshort{Laws}	\gdef\@journalfull{Laws}	\gdef\@doiabbr{laws}	\gdef\@ISSN{2075-471X}	}
\DeclareOption{life}{	\gdef\@journal{life}	\gdef\@journalshort{Life}	\gdef\@journalfull{Life}	\gdef\@doiabbr{life}	\gdef\@ISSN{2075-1729}	}
\DeclareOption{literature}{	\gdef\@journal{literature}	\gdef\@journalshort{Literature}	\gdef\@journalfull{Literature}	\gdef\@doiabbr{}	\gdef\@ISSN{2410-9789}	}
\DeclareOption{logistics}{	\gdef\@journal{logistics}	\gdef\@journalshort{Logistics}	\gdef\@journalfull{Logistics}	\gdef\@doiabbr{logistics}	\gdef\@ISSN{2305-6290}	}
\DeclareOption{lubricants}{	\gdef\@journal{lubricants}	\gdef\@journalshort{Lubricants}	\gdef\@journalfull{Lubricants}	\gdef\@doiabbr{lubricants}	\gdef\@ISSN{2075-4442}	}
\DeclareOption{machines}{	\gdef\@journal{machines}	\gdef\@journalshort{Machines}	\gdef\@journalfull{Machines}	\gdef\@doiabbr{machines}	\gdef\@ISSN{2075-1702}	}
\DeclareOption{magnetochemistry}{	\gdef\@journal{magnetochemistry}	\gdef\@journalshort{Magnetochemistry}	\gdef\@journalfull{Magnetochemistry}	\gdef\@doiabbr{magnetochemistry}	\gdef\@ISSN{2312-7481}	}
\DeclareOption{make}{	\gdef\@journal{make}	\gdef\@journalshort{Mach. Learn. Knowl. Extr.}	\gdef\@journalfull{Machine Learning and Knowledge Extraction}	\gdef\@doiabbr{make}	\gdef\@ISSN{2504-4990}	}
\DeclareOption{marinedrugs}{	\gdef\@journal{marinedrugs}	\gdef\@journalshort{Mar. Drugs}	\gdef\@journalfull{Marine Drugs}	\gdef\@doiabbr{md}	\gdef\@ISSN{1660-3397}	}
\DeclareOption{materials}{	\gdef\@journal{materials}	\gdef\@journalshort{Materials}	\gdef\@journalfull{Materials}	\gdef\@doiabbr{ma}	\gdef\@ISSN{1996-1944}	}
\DeclareOption{mathematics}{	\gdef\@journal{mathematics}	\gdef\@journalshort{Mathematics}	\gdef\@journalfull{Mathematics}	\gdef\@doiabbr{math}	\gdef\@ISSN{2227-7390}	}
\DeclareOption{mca}{	\gdef\@journal{mca}	\gdef\@journalshort{Math. Comput. Appl.}	\gdef\@journalfull{Mathematical and Computational Applications}	\gdef\@doiabbr{mca}	\gdef\@ISSN{2297-8747}	}
\DeclareOption{medicina}{	\gdef\@journal{medicina}	\gdef\@journalshort{Medicina}	\gdef\@journalfull{Medicina}	\gdef\@doiabbr{medicina}	\gdef\@ISSN{1010-660X}	}
\DeclareOption{medicines}{	\gdef\@journal{medicines}	\gdef\@journalshort{Medicines}	\gdef\@journalfull{Medicines}	\gdef\@doiabbr{medicines}	\gdef\@ISSN{2305-6320}	}
\DeclareOption{medsci}{	\gdef\@journal{medsci}	\gdef\@journalshort{Med. Sci.}	\gdef\@journalfull{Medical Sciences}	\gdef\@doiabbr{medsci}	\gdef\@ISSN{2076-3271}	}
\DeclareOption{membranes}{	\gdef\@journal{membranes}	\gdef\@journalshort{Membranes}	\gdef\@journalfull{Membranes}	\gdef\@doiabbr{membranes}	\gdef\@ISSN{2077-0375}	}
\DeclareOption{metabolites}{	\gdef\@journal{metabolites}	\gdef\@journalshort{Metabolites}	\gdef\@journalfull{Metabolites}	\gdef\@doiabbr{metabo}	\gdef\@ISSN{2218-1989}	}
\DeclareOption{metals}{	\gdef\@journal{metals}	\gdef\@journalshort{Metals}	\gdef\@journalfull{Metals}	\gdef\@doiabbr{met}	\gdef\@ISSN{2075-4701}	}
\DeclareOption{microarrays}{	\gdef\@journal{microarrays}	\gdef\@journalshort{Microarrays}	\gdef\@journalfull{Microarrays}	\gdef\@doiabbr{}	\gdef\@ISSN{2076-3905}	}
\DeclareOption{micromachines}{	\gdef\@journal{micromachines}	\gdef\@journalshort{Micromachines}	\gdef\@journalfull{Micromachines}	\gdef\@doiabbr{mi}	\gdef\@ISSN{2072-666X}	}
\DeclareOption{microorganisms}{	\gdef\@journal{microorganisms}	\gdef\@journalshort{Microorganisms}	\gdef\@journalfull{Microorganisms}	\gdef\@doiabbr{microorganisms}	\gdef\@ISSN{2076-2607}	}
\DeclareOption{minerals}{	\gdef\@journal{minerals}	\gdef\@journalshort{Minerals}	\gdef\@journalfull{Minerals}	\gdef\@doiabbr{min}	\gdef\@ISSN{2075-163X}	}
\DeclareOption{modelling}{	\gdef\@journal{modelling}	\gdef\@journalshort{Modelling}	\gdef\@journalfull{Modelling}	\gdef\@doiabbr{}	\gdef\@ISSN{0012-0012}	}
\DeclareOption{molbank}{	\gdef\@journal{molbank}	\gdef\@journalshort{Molbank}	\gdef\@journalfull{Molbank}	\gdef\@doiabbr{M}	\gdef\@ISSN{1422-8599}	}
\DeclareOption{molecules}{	\gdef\@journal{molecules}	\gdef\@journalshort{Molecules}	\gdef\@journalfull{Molecules}	\gdef\@doiabbr{molecules}	\gdef\@ISSN{1420-3049}	}
\DeclareOption{mps}{	\gdef\@journal{mps}	\gdef\@journalshort{Methods and Protoc.}	\gdef\@journalfull{Methods and Protocols}	\gdef\@doiabbr{mps}	\gdef\@ISSN{2409-9279}	}
\DeclareOption{mti}{	\gdef\@journal{mti}	\gdef\@journalshort{Multimodal Technologies and Interact.}	\gdef\@journalfull{Multimodal Technologies and Interaction}	\gdef\@doiabbr{mti}	\gdef\@ISSN{2414-4088}	}
\DeclareOption{nanomaterials}{	\gdef\@journal{nanomaterials}	\gdef\@journalshort{Nanomaterials}	\gdef\@journalfull{Nanomaterials}	\gdef\@doiabbr{nano}	\gdef\@ISSN{2079-4991}	}
\DeclareOption{ncrna}{	\gdef\@journal{ncrna}	\gdef\@journalshort{Non-coding RNA}	\gdef\@journalfull{Non-coding RNA}	\gdef\@doiabbr{ncrna}	\gdef\@ISSN{2311-553X}	}
\DeclareOption{neonatalscreening}{	\gdef\@journal{neonatalscreening}	\gdef\@journalshort{Int. J. Neonatal Screen.}	\gdef\@journalfull{International Journal of Neonatal Screening}	\gdef\@doiabbr{ijns}	\gdef\@ISSN{2409-515X}	}
\DeclareOption{neuroglia}{	\gdef\@journal{neuroglia}	\gdef\@journalshort{Neuroglia}	\gdef\@journalfull{Neuroglia}	\gdef\@doiabbr{neuroglia}	\gdef\@ISSN{2571-6980}	}
\DeclareOption{nitrogen}{	\gdef\@journal{nitrogen}	\gdef\@journalshort{Nitrogen}	\gdef\@journalfull{Nitrogen}	\gdef\@doiabbr{nitrogen}	\gdef\@ISSN{2504-3129}	}
\DeclareOption{notspecified}{	\gdef\@journal{notspecified}	\gdef\@journalshort{Journal Not Specified}	\gdef\@journalfull{Journal Not Specified}	\gdef\@doiabbr{}	\gdef\@ISSN{}	}
\DeclareOption{nutrients}{	\gdef\@journal{nutrients}	\gdef\@journalshort{Nutrients}	\gdef\@journalfull{Nutrients}	\gdef\@doiabbr{nu}	\gdef\@ISSN{2072-6643}	}
\DeclareOption{ohbm}{	\gdef\@journal{ohbm}	\gdef\@journalshort{J. Otorhinolaryngol. Hear. Balance Med.}	"\gdef\@journalfull{Journal of Otorhinolaryngology, Hearing and Balance Medicine}"	\gdef\@doiabbr{ohbm}	\gdef\@ISSN{2504-463X}	}
\DeclareOption{particles}{	\gdef\@journal{particles}	\gdef\@journalshort{Particles}	\gdef\@journalfull{Particles}	\gdef\@doiabbr{particles}	\gdef\@ISSN{2571-712X}	}
\DeclareOption{pathogens}{	\gdef\@journal{pathogens}	\gdef\@journalshort{Pathogens}	\gdef\@journalfull{Pathogens}	\gdef\@doiabbr{pathogens}	\gdef\@ISSN{2076-0817}	}
\DeclareOption{pharmaceuticals}{	\gdef\@journal{pharmaceuticals}	\gdef\@journalshort{Pharmaceuticals}	\gdef\@journalfull{Pharmaceuticals}	\gdef\@doiabbr{ph}	\gdef\@ISSN{1424-8247}	}
\DeclareOption{pharmaceutics}{	\gdef\@journal{pharmaceutics}	\gdef\@journalshort{Pharmaceutics}	\gdef\@journalfull{Pharmaceutics}	\gdef\@doiabbr{pharmaceutics}	\gdef\@ISSN{1999-4923}	}
\DeclareOption{pharmacy}{	\gdef\@journal{pharmacy}	\gdef\@journalshort{Pharmacy}	\gdef\@journalfull{Pharmacy}	\gdef\@doiabbr{pharmacy}	\gdef\@ISSN{2226-4787}	}
\DeclareOption{philosophies}{	\gdef\@journal{philosophies}	\gdef\@journalshort{Philosophies}	\gdef\@journalfull{Philosophies}	\gdef\@doiabbr{philosophies}	\gdef\@ISSN{2409-9287}	}
\DeclareOption{photonics}{	\gdef\@journal{photonics}	\gdef\@journalshort{Photonics}	\gdef\@journalfull{Photonics}	\gdef\@doiabbr{photonics}	\gdef\@ISSN{2304-6732}	}
\DeclareOption{plants}{	\gdef\@journal{plants}	\gdef\@journalshort{Plants}	\gdef\@journalfull{Plants}	\gdef\@doiabbr{plants}	\gdef\@ISSN{2223-7747}	}
\DeclareOption{plasma}{	\gdef\@journal{plasma}	\gdef\@journalshort{Plasma}	\gdef\@journalfull{Plasma}	\gdef\@doiabbr{plasma}	\gdef\@ISSN{2571-6182}	}
\DeclareOption{polymers}{	\gdef\@journal{polymers}	\gdef\@journalshort{Polymers}	\gdef\@journalfull{Polymers}	\gdef\@doiabbr{polym}	\gdef\@ISSN{2073-4360}	}
\DeclareOption{polysaccharides}{	\gdef\@journal{polysaccharides}	\gdef\@journalshort{Polysaccharides}	\gdef\@journalfull{Polysaccharides}	\gdef\@doiabbr{}	\gdef\@ISSN{}	}
\DeclareOption{preprints}{ 	\gdef\@journal{preprints} 	\gdef\@journalshort{Preprints}	\gdef\@journalfull{Preprints}	\gdef\@doiabbr{}	\gdef\@ISSN{}	}
\DeclareOption{proceedings}{	\gdef\@journal{proceedings}	\gdef\@journalshort{Proceedings}	\gdef\@journalfull{Proceedings}	\gdef\@doiabbr{proceedings}	\gdef\@ISSN{2504-3900}	}
\DeclareOption{processes}{	\gdef\@journal{processes}	\gdef\@journalshort{Processes}	\gdef\@journalfull{Processes}	\gdef\@doiabbr{pr}	\gdef\@ISSN{2227-9717}	}
\DeclareOption{proteomes}{	\gdef\@journal{proteomes}	\gdef\@journalshort{Proteomes}	\gdef\@journalfull{Proteomes}	\gdef\@doiabbr{proteomes}	\gdef\@ISSN{2227-7382}	}
\DeclareOption{publications}{	\gdef\@journal{publications}	\gdef\@journalshort{Publications}	\gdef\@journalfull{Publications}	\gdef\@doiabbr{publications}	\gdef\@ISSN{2304-6775}	}
\DeclareOption{quantumrep}{	\gdef\@journal{quantumrep}	\gdef\@journalshort{Quantum Rep.}	\gdef\@journalfull{Quantum Reports}	\gdef\@doiabbr{}	\gdef\@ISSN{}	}
\DeclareOption{quaternary}{	\gdef\@journal{quaternary}	\gdef\@journalshort{Quaternary}	\gdef\@journalfull{Quaternary}	\gdef\@doiabbr{quat}	\gdef\@ISSN{2571-550X}	}
\DeclareOption{qubs}{	\gdef\@journal{qubs}	\gdef\@journalshort{Quantum Beam Sci.}	\gdef\@journalfull{Quantum Beam Science}	\gdef\@doiabbr{qubs}	\gdef\@ISSN{2412-382X}	}
\DeclareOption{reactions}{	\gdef\@journal{reactions}	\gdef\@journalshort{Reactions}	\gdef\@journalfull{Reactions}	\gdef\@doiabbr{reactions}	\gdef\@ISSN{2624-781X}	}
\DeclareOption{recycling}{	\gdef\@journal{recycling}	\gdef\@journalshort{Recycling}	\gdef\@journalfull{Recycling}	\gdef\@doiabbr{recycling}	\gdef\@ISSN{2313-4321}	}
\DeclareOption{religions}{	\gdef\@journal{religions}	\gdef\@journalshort{Religions}	\gdef\@journalfull{Religions}	\gdef\@doiabbr{rel}	\gdef\@ISSN{2077-1444}	}
\DeclareOption{remotesensing}{	\gdef\@journal{remotesensing}	\gdef\@journalshort{Remote Sens.}	\gdef\@journalfull{Remote Sensing}	\gdef\@doiabbr{rs}	\gdef\@ISSN{2072-4292}	}
\DeclareOption{reports}{	\gdef\@journal{reports}	\gdef\@journalshort{Reports}	\gdef\@journalfull{Reports}	\gdef\@doiabbr{reports}	\gdef\@ISSN{2571-841X}	}
\DeclareOption{resources}{	\gdef\@journal{resources}	\gdef\@journalshort{Resources}	\gdef\@journalfull{Resources}	\gdef\@doiabbr{resources}	\gdef\@ISSN{2079-9276}	}
\DeclareOption{risks}{	\gdef\@journal{risks}	\gdef\@journalshort{Risks}	\gdef\@journalfull{Risks}	\gdef\@doiabbr{risks}	\gdef\@ISSN{2227-9091}	}
\DeclareOption{robotics}{	\gdef\@journal{robotics}	\gdef\@journalshort{Robotics}	\gdef\@journalfull{Robotics}	\gdef\@doiabbr{robotics}	\gdef\@ISSN{2218-6581}	}
\DeclareOption{safety}{	\gdef\@journal{safety}	\gdef\@journalshort{Safety}	\gdef\@journalfull{Safety}	\gdef\@doiabbr{safety}	\gdef\@ISSN{2313-576X}	}
\DeclareOption{sci}{	\gdef\@journal{sci}	\gdef\@journalshort{Sci}	\gdef\@journalfull{Sci}	\gdef\@doiabbr{sci}	\gdef\@ISSN{2413-4155}	}
\DeclareOption{scipharm}{	\gdef\@journal{scipharm}	\gdef\@journalshort{Sci. Pharm.}	\gdef\@journalfull{Scientia Pharmaceutica}	\gdef\@doiabbr{scipharm}	\gdef\@ISSN{2218-0532}	}
\DeclareOption{sensors}{	\gdef\@journal{sensors}	\gdef\@journalshort{Sensors}	\gdef\@journalfull{Sensors}	\gdef\@doiabbr{s}	\gdef\@ISSN{1424-8220}	}
\DeclareOption{separations}{	\gdef\@journal{separations}	\gdef\@journalshort{Separations}	\gdef\@journalfull{Separations}	\gdef\@doiabbr{separations}	\gdef\@ISSN{2297-8739}	}
\DeclareOption{sexes}{	\gdef\@journal{sexes}	\gdef\@journalshort{Sexes}	\gdef\@journalfull{Sexes}	\gdef\@doiabbr{}	\gdef\@ISSN{2411-5118}	}
\DeclareOption{signals}{	\gdef\@journal{signals}	\gdef\@journalshort{Signals}	\gdef\@journalfull{Signals}	\gdef\@doiabbr{signals}	\gdef\@ISSN{2624-6120}	}
\DeclareOption{sinusitis}{	\gdef\@journal{sinusitis}	\gdef\@journalshort{Sinusitis}	\gdef\@journalfull{Sinusitis}	\gdef\@doiabbr{sinusitis}	\gdef\@ISSN{2309-107X}	}
\DeclareOption{smartcities}{	\gdef\@journal{smartcities}	\gdef\@journalshort{Smart Cities}	\gdef\@journalfull{Smart Cities}	\gdef\@doiabbr{smartcities}	\gdef\@ISSN{}	}
\DeclareOption{societies}{	\gdef\@journal{societies}	\gdef\@journalshort{Societies}	\gdef\@journalfull{Societies}	\gdef\@doiabbr{soc}	\gdef\@ISSN{2075-4698}	}
\DeclareOption{socsci}{	\gdef\@journal{socsci}	\gdef\@journalshort{Soc. Sci.}	\gdef\@journalfull{Social Sciences}	\gdef\@doiabbr{socsci}	\gdef\@ISSN{2076-0760}	}
\DeclareOption{soilsystems}{	\gdef\@journal{soilsystems}	\gdef\@journalshort{Soil Syst.}	\gdef\@journalfull{Soil Systems}	\gdef\@doiabbr{soilsystems}	\gdef\@ISSN{2571-8789}	}
\DeclareOption{sports}{	\gdef\@journal{sports}	\gdef\@journalshort{Sports}	\gdef\@journalfull{Sports}	\gdef\@doiabbr{sports}	\gdef\@ISSN{2075-4663}	}
\DeclareOption{standards}{	\gdef\@journal{standards}	\gdef\@journalshort{Standards}	\gdef\@journalfull{Standards}	\gdef\@doiabbr{}	\gdef\@ISSN{2305-6703}	}
\DeclareOption{stats}{	\gdef\@journal{stats}	\gdef\@journalshort{Stats}	\gdef\@journalfull{Stats}	\gdef\@doiabbr{stats}	\gdef\@ISSN{2571-905X}	}
\DeclareOption{surfaces}{	\gdef\@journal{surfaces}	\gdef\@journalshort{Surfaces}	\gdef\@journalfull{Surfaces}	\gdef\@doiabbr{surfaces}	\gdef\@ISSN{2571-9637}	}
\DeclareOption{surgeries}{	\gdef\@journal{surgeries}	\gdef\@journalshort{Surgeries}	\gdef\@journalfull{Surgeries}	\gdef\@doiabbr{}	\gdef\@ISSN{2017-2017}	}
\DeclareOption{sustainability}{	\gdef\@journal{sustainability}	\gdef\@journalshort{Sustainability}	\gdef\@journalfull{Sustainability}	\gdef\@doiabbr{su}	\gdef\@ISSN{2071-1050}	}
\DeclareOption{symmetry}{	\gdef\@journal{symmetry}	\gdef\@journalshort{Symmetry}	\gdef\@journalfull{Symmetry}	\gdef\@doiabbr{sym}	\gdef\@ISSN{2073-8994}	}
\DeclareOption{systems}{	\gdef\@journal{systems}	\gdef\@journalshort{Systems}	\gdef\@journalfull{Systems}	\gdef\@doiabbr{systems}	\gdef\@ISSN{2079-8954}	}
\DeclareOption{technologies}{	\gdef\@journal{technologies}	\gdef\@journalshort{Technologies}	\gdef\@journalfull{Technologies}	\gdef\@doiabbr{technologies}	\gdef\@ISSN{2227-7080}	}
\DeclareOption{test}{	\gdef\@journal{test}	\gdef\@journalshort{Test}	\gdef\@journalfull{Test}	\gdef\@doiabbr{}	\gdef\@ISSN{}	}
\DeclareOption{toxics}{	\gdef\@journal{toxics}	\gdef\@journalshort{Toxics}	\gdef\@journalfull{Toxics}	\gdef\@doiabbr{toxics}	\gdef\@ISSN{2305-6304}	}
\DeclareOption{toxins}{	\gdef\@journal{toxins}	\gdef\@journalshort{Toxins}	\gdef\@journalfull{Toxins}	\gdef\@doiabbr{toxins}	\gdef\@ISSN{2072-6651}	}
\DeclareOption{tropicalmed}{	\gdef\@journal{tropicalmed}	\gdef\@journalshort{Trop. Med. Infect. Dis.}	\gdef\@journalfull{Tropical Medicine and Infectious Disease}	\gdef\@doiabbr{tropicalmed}	\gdef\@ISSN{2414-6366}	}
\DeclareOption{universe}{	\gdef\@journal{universe}	\gdef\@journalshort{Universe}	\gdef\@journalfull{Universe}	\gdef\@doiabbr{universe}	\gdef\@ISSN{2218-1997}	}
\DeclareOption{urbansci}{	\gdef\@journal{urbansci}	\gdef\@journalshort{Urban Sci.}	\gdef\@journalfull{Urban Science}	\gdef\@doiabbr{urbansci}	\gdef\@ISSN{2413-8851}	}
\DeclareOption{vaccines}{	\gdef\@journal{vaccines}	\gdef\@journalshort{Vaccines}	\gdef\@journalfull{Vaccines}	\gdef\@doiabbr{vaccines}	\gdef\@ISSN{2076-393X}	}
\DeclareOption{vehicles}{	\gdef\@journal{vehicles}	\gdef\@journalshort{Vehicles}	\gdef\@journalfull{Vehicles}	\gdef\@doiabbr{}	\gdef\@ISSN{}	}
\DeclareOption{vetsci}{	\gdef\@journal{vetsci}	\gdef\@journalshort{Vet. Sci.}	\gdef\@journalfull{Veterinary Sciences}	\gdef\@doiabbr{vetsci}	\gdef\@ISSN{2306-7381}	}
\DeclareOption{vibration}{	\gdef\@journal{vibration}	\gdef\@journalshort{Vibration}	\gdef\@journalfull{Vibration}	\gdef\@doiabbr{vibration}	\gdef\@ISSN{2571-631X}	}
\DeclareOption{viruses}{	\gdef\@journal{viruses}	\gdef\@journalshort{Viruses}	\gdef\@journalfull{Viruses}	\gdef\@doiabbr{v}	\gdef\@ISSN{1999-4915}	}
\DeclareOption{vision}{	\gdef\@journal{vision}	\gdef\@journalshort{Vision}	\gdef\@journalfull{Vision}	\gdef\@doiabbr{vision}	\gdef\@ISSN{2411-5150}	}
\DeclareOption{water}{	\gdef\@journal{water}	\gdef\@journalshort{Water}	\gdef\@journalfull{Water}	\gdef\@doiabbr{w}	\gdef\@ISSN{2073-4441}	}
\DeclareOption{wem}{	\gdef\@journal{wem}	\gdef\@journalshort{Wildl. Ecol. Manag.}	\gdef\@journalfull{Wildlife Ecology and Management}	\gdef\@doiabbr{}	\gdef\@ISSN{1234-4321}	}
\DeclareOption{wevj}{	\gdef\@journal{wevj}	\gdef\@journalshort{World Electric Vehicle Journal}	\gdef\@journalfull{World Electric Vehicle Journal}	\gdef\@doiabbr{wevj}	\gdef\@ISSN{2032-6653}	}
